Discovery prospects for long-lived multiply charged particles at the LHC

In this work, we aim to provide a comprehensive and largely model independent investigation on prospects to detect long-lived multiply charged particles at the LHC. We consider particles with spin 0 and $\frac{1}{2}$, with electric charges in range $1 \le |Q/e| \le 8$, which are singlet or triplet under $SU(3)_C$. Such particles might be produced as particle-antiparticle pairs and propagate through detectors, or form a positronium(quarkonium)-like bound state. We consider both possibilities and estimate lower mass bounds on new particles, that can be provided by ATLAS, CMS and MoEDAL experiments at the end of Run 3 and HL-LHC data taking periods. We find out that the sensitivities of ATLAS and CMS are generally stronger than those of MoEDAL at Run 3, while they may be competitive at HL-LHC for $3 \lesssim |Q/e| \lesssim 7$ for all types of long-lived particles we consider.

==> Highly charged LLP at MoEDAL (Version 7545)/cfHighQ_reach.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q1.pdf} \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q2.pdf}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q3.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q4.pdf}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q5.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q6.pdf}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q7.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/cfHighQ/reach_Q8.pdf}  
\caption{\small Model-independent detection reach at MoEDAL in the ($m$, $c
  \tau$) parameter plane for coloured fermions. The
  solid dashed and dotted contours correspond to $N_{\rm sig} = 1$, 2
  and 3, respectively. Green and red contours correspond to Run-3 
  $(L=30$ $\mathrm{fb}{}^{-1})$ and HL-LHC $(L=300$ $\mathrm{fb}^{-1})$ luminosities respectively.
  }
\label{fig:lim_cfHighQ}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	

==> Highly charged LLP at MoEDAL (Version 7545)/csHighQ_reach.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q1.pdf} \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q2.pdf}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q3.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q4.pdf}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q5.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q6.pdf}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q7.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/csHighQ/reach_Q8.pdf}  
\caption{\small Model-independent detection reach at MoEDAL in the ($m$, $c
  \tau$) parameter plane for coloured scalars. The
  solid dashed and dotted contours correspond to $N_{\rm sig} = 1$, 2
  and 3, respectively. Green and red contours correspond to Run-3 
  $(L=30$ $\mathrm{fb}{}^{-1})$ and HL-LHC $(L=300$ $\mathrm{fb}^{-1})$ luminosities respectively.
  }
\label{fig:lim_csHighQ}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	

==> Highly charged LLP at MoEDAL (Version 7545)/fHighQ_reach.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q1.pdf} \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q2.pdf}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q3.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q4.pdf}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q5.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q6.pdf}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q7.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/fHighQ/reach_Q8.pdf}  
\caption{\small Model-independent detection reach at MoEDAL in the ($m$, $c
  \tau$) parameter plane for colourless fermions. The
  solid dashed and dotted contours correspond to $N_{\rm sig} = 1$, 2
  and 3, respectively. Green and red contours correspond to Run-3 
  $(L=30$ $\mathrm{fb}{}^{-1})$ and HL-LHC $(L=300$ $\mathrm{fb}^{-1})$ luminosities respectively.
  }
\label{fig:lim_fHighQ}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	

==> Highly charged LLP at MoEDAL (Version 7545)/sHighQ_reach.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q1.pdf} \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q2.pdf}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q3.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q4.pdf}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q5.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q6.pdf}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q7.pdf}  \hspace{5mm}
      \includegraphics[width=0.4\textwidth]{figs/sHighQ/reach_Q8.pdf}  
\caption{\small Model-independent detection reach at MoEDAL in the ($m$, $c
  \tau$) parameter plane for colourless scalars. The
  solid dashed and dotted contours correspond to $N_{\rm sig} = 1$, 2
  and 3, respectively. Green and red contours correspond to Run-3 
  $(L=30$ $\mathrm{fb}{}^{-1})$ and HL-LHC $(L=300$ $\mathrm{fb}^{-1})$ luminosities respectively.
  }
\label{fig:lim_sHighQ}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
